A burst search for gravitational waves from binary black holes

Compact binary coalescence (CBC) is one of the most promising sources of gravitational waves. These sources are usually searched for with matched filters which require accurate calculation of the GW waveforms and generation of large template banks. We present a complementary search technique based on algorithms used in un-modeled searches. Initially designed for detection of un-modeled bursts, which can span a very large set of waveform morphologies, the search algorithm presented here is constrained for targeted detection of the smaller subset of CBC signals. The constraint is based on the assumption of elliptical polarisation for signals received at the detector. We expect that the algorithm is sensitive to CBC signals in a wide range of masses, mass ratios, and spin parameters. In preparation for the analysis of data from the fifth LIGO-Virgo science run (S5), we performed preliminary studies of the algorithm on test data. We present the sensitivity of the search to different types of simulated CBC waveforms. Also, we discuss how to extend the results of the test run into a search over all of the current LIGO-Virgo data set.

==> references.tex <==
	
		
@article{Klimenko:2005wa,
	Author = {S. Klimenko and S. Mohanty and M. Rakhmanov and G. Mitselmakher},
	Date-Added = {2007-10-28 10:44:21 -0400},
	Date-Modified = {2007-10-28 11:01:50 -0400},
	Journal = {Physical Review D},
	Keywords = {network, likelihood, constraint, ligo, interferometer},
	Month = {December},
	Read = {Yes},
	Title = {Constraint likelihood analysis for a network of gravitational wave detectors},
	Volume = {72},
        Pages = {122002},
	Year = {2005}}

@article{Klimenko:2006io,
	Author = {S. Klimenko and S. Mohanty and M. Rakhmanov and G. Mitselmakher},
	Date-Added = {2009-03-16 16:14:30 -0700},
	Date-Modified = {2009-03-16 16:15:37 -0700},
	Journal = {Journal of Physics},
	Number = {1},
	Title = {Constraint likelihood method: generalization for colored noise},
	Volume = {32},
        Pages = {12-17},
	Year = {2006}}

@article{Klimenko:2007hd,
	Author = {S. Klimenko and I. Yakushin and A. Mercer and G. Mitselmakher},
	Date-Added = {2007-12-19 00:26:14 -0500},
	Date-Modified = {2008-04-02 14:47:41 -0400},
	Journal = {arXiv:0802.3232v2 [gr-qc]},
	Read = {Yes},
	Title = {Coherent algorithm for detection of gravitational wave bursts},
        Pages = {114029},
	Year = {2008}}
	
@article{Damour:2008lu,
	Author = {Thibault Damour and Alessandro Nagar and Ernst Nils Dorband and Denis Pollney and Luciano Rezzolla},
	Date-Added = {2007-12-28 16:09:24 -0500},
	Date-Modified = {2007-12-28 16:11:26 -0500},
	Journal = {Phys. Rev. D},
	Title = {Faithful Effective-One-Body waveforms of equal-mass coalescing black-hole binaries},
	Volume = {2008},
        Pages = {084017},
	Year = {2008}}


@article{Kopparapu:2007kx,
	Author = {Kumar Kopparapu and Chad Hanna and Viky Kalogera and Richard O'Shaughnessy and Gabriela Gonzalez, Patrick R. Brady, Stephen Fairhurst},
	Date-Added = {2008-03-15 15:08:26 -0400},
	Date-Modified = {2009-04-03 12:42:06 -0400},
	Journal = {Astrophysical Journal},
	Month = {March},
	Title = {Host Galaxies Catalog Used in LIGO Searches for Compact Binary Coalescence Events},
        Volume = {675},
        Number = {2},
        Pages = {1459-1467},
	Year = {2008}}


@inproceedings{Blanchet:2001og,
	Author = {Luc Blanchet},
	Booktitle = {Gravitatonal Waves, Proceedings of the Como School on Gravitational Waves in Astrophysics},
	Date-Added = {2008-04-02 14:41:28 -0400},
	Date-Modified = {2008-04-02 14:43:25 -0400},
	Editor = {I. Ciufolini and V. Gorini and U. Moschella and P. Fre},
	Publisher = {Institute of Physics Publishing},
	Title = {Post-Newtonian Computation of Binary Inspiral Waveforms},
	Year = {2001}}
	
@article{Abbot:2007uq,
	Author = {B. Abbot and others},
	Date-Added = {2008-01-28 17:01:20 -0500},
	Date-Modified = {2008-01-28 17:02:11 -0500},
	Journal = {Physical Review D},
	Read = {Yes},
	Title = {Search for gravitational waves from binary inspirals in S3 and S4 LIGO data},
        Volume = {77},
        Number = {6},
        Pages = {062002},
	Year = {2007}}
	
@article{Abbott:2008eh,
	Author = {B. Abbott and others},
	Date-Added = {2009-03-16 15:24:39 -0700},
	Date-Modified = {2009-03-16 15:31:09 -0700},
	Journal = {Class. Quant. Grav.},
	Month = {December},
	Title = {First joint search for gravitational-wave bursts in LIGO and GEO600 data},
	Volume = {25},
        Number = {24},
        Pages = {245008},
	Year = {2008}}


@article{Pai:2004rf,
	Author = {Sukanta Bose and Archana Pai and Sanjeev Dhurandhar},
	Date-Added = {2009-03-16 15:32:50 -0700},
	Date-Modified = {2009-03-16 15:34:31 -0700},
	Journal = {Phys. Rev. D},
	Pages = {042004},
	Title = {A data-analysis strategy for detecting gravitational-wave signals from inspiraling compact binaries with a network of laser-interferometric detectors},
	Volume = {64},
	Year = {2001}}

@article{Tagoshi:2008ij,
	Author = {Hideyuki Tagoshi and Himan Mukhopadhyay and Sanjeev Dhurandhar and Norichika Sago and Hirotaka Takahashi and Nobuyuki Kanda},
	Date-Added = {2009-03-16 16:00:05 -0700},
	Date-Modified = {2009-03-16 16:03:49 -0700},
	Journal = {Phys. Rev. D},
	Number = {8},
	Pages = {083005},
	Title = {Detecting gravitational waves from inspiraling binaries with a network of detectors : coherent strategies by correlated detectors},
	Volume = {75},
	Year = {2007}}
	
	
@article{Buonanno:2007qm,
	Author = {Alessandra Buonanno and Gregory B. Cook and Frans Pretorius},
	Date-Added = {2009-03-23 12:46:47 -0400},
	Date-Modified = {2009-03-23 12:52:21 -0400},
	Journal = {Phys. Rev. D},
	Number = {12},
	Read = {Yes},
	Title = {Inspiral, merger and ring-down of equal-mass black-hole binaries},
	Volume = {75},
        Pages = {123018},
	Year = {2007}}

	

@article{Ajith:2007fj,
	Author = {P. Ajith and others},
	Date-Added = {2008-01-28 17:02:18 -0500},
	Date-Modified = {2009-03-23 12:56:00 -0400},
	Journal = {Phys. Rev. D},
	Month = {May},
	Number = {10},
	Read = {Yes},
	Title = {A template bank for gravitational waveforms form coalescing binary black holes: I. non-spinning binaries},
	Volume = {77},
        Pages = {04017},
	Year = {2008}}


@article{Buonanno:2003nw,
	Author = {Alessandra Buonanno and Yanbei Chan and Michele Vallisneri},
	Date-Added = {2009-03-23 14:08:13 -0400},
	Date-Modified = {2009-03-23 14:14:31 -0400},
	Journal = {Phys. Rev. D},
	Read = {Yes},
	Title = {Detecting gravitational waves from precessing binaries of spinning compact objects: Adabatic limit},
	Volume = {67},
        Pages = {104025},
	Year = {2003}}


@article{Pan:2003br,
	Author = {Yi Pan and Alessandra Buonanno and Yanbei Chan and Michele Vallisneri},
	Date-Added = {2009-03-23 14:20:08 -0400},
	Date-Modified = {2009-03-23 14:21:01 -0400},
	Journal = {Phys. Rev. D},
	Title = {A physical template family for gravitational waves from precessing binaries of spinning compact objects: Application to single-spin binaries},
	Volume = {69},
        Pages = {104017},
	Year = {2003}}


@article{Buonanno:2004zb,
	Author = {Alessandra Buonanno and Yanbei Chan and Michele Vallisneri},
	Date-Added = {2009-03-23 14:18:02 -0400},
	Date-Modified = {2009-03-23 14:21:22 -0400},
	Journal = {Phys. Rev. D},
	Title = {A quasi-physical family of gravity-wave templates for precessing binaries of spinning compact objects: Application to double-spin precessing binaries},
	Volume = {70},
        Pages = {104003},
	Year = {2004}}
	
	
@article{Buonanno:1999sp,
	Author = {A. Buonanno and T. Damour},
	Date-Added = {2009-03-23 14:31:05 -0400},
	Date-Modified = {2009-03-23 14:31:48 -0400},
	Journal = {Phys. Rev. D},
	Title = {Effective one-body approach to general relativistic two-body dynamics},
	Volume = {D59},
        Pages = {084006},
	Year = {1999}}


@article{Gusel:1989dd,
	Author = {Yekta G\"{u}sel and Massimo Tinto},
	Date-Added = {2009-03-23 14:46:09 -0400},
	Date-Modified = {2009-03-23 14:48:21 -0400},
	Journal = {Phys. Rev. D},
	Number = {12},
	Title = {Near optimal solution to the inverse problem for gravitational-wave bursts},
	Volume = {40},
        Pages = {3884-3938},
	Year = {1989}}


@article{Anderson:2006dg,
	Author = {Warren G. Anderson and Patrick R. Brady and Jolien D. E. Creighton and \'{E}anna \'{E} Flanagan},
	Date-Added = {2009-03-23 14:59:35 -0400},
	Date-Modified = {2009-03-23 15:02:21 -0400},
	Journal = {Phys. Rev. D},
	Number = {4},
	Title = {An excess power statistic for detection of burst sources of gravitational radiation},
	Volume = {63},
        Pages = {042003},
	Year = {2000}}

@article{Chatterji:2004mv,
	Author = {S. Chatterji and L. Blackburn and G. Martin and E. Katsavounidis},
	Date-Added = {2007-12-28 16:00:02 -0500},
	Date-Modified = {2009-08-14 10:34:09 -0400},
	Journal = {Class. Quant. Grav.},
	Month = {October},
	Number = {20},
	Pages = {S1809-S1818},
	Title = {Multiresolution techniques for the detection of gravitational-wave bursts},
	Url = {arXiv:gr-qc/0412119v1},
	Volume = {21},
	Year = {2004},
	Bdsk-Url-1 = {arXiv:gr-qc/0412119v1}}

@article{Arnaud:2003ts,
	Author = {Nicolas Arnaud and Matteo Barsuglia and Marie-Anne Bizouard and Violette Brisson and Fabien Cavalier and Michel Davier and Patrice Hello and Stephane Kreckelbergh and Edward K. Porter},
	Date-Added = {2009-03-23 15:15:49 -0400},
	Date-Modified = {2009-03-23 15:18:10 -0400},
	Journal = {Phys. Rev. D},
	Title = {Coincidence and coherent data analysis methods for gravitational wave bursts in a network of interferometer detectors},
	Volume = {68},
        Pages = {102001},
	Year = {2003}}


@book{Binney:1998qm,
	Author = {James Binney and Michael Merrifield},
	Date-Added = {2009-03-26 09:45:30 -0400},
	Date-Modified = {2009-03-26 09:46:39 -0400},
	Publisher = {Princeton University Press},
	Title = {Galactic Astronomy},
	Year = {1998}}


@article{Sathyaprakash:1999cw,
	Author = {B. S. Sathyaprakash and S. V. Dhurandhar},
	Date-Added = {2009-03-26 14:21:30 -0400},
	Date-Modified = {2009-03-26 14:32:33 -0400},
	Journal = {Phys. Rev. D},
	Number = {12},
	Title = {Choice of filters for the detection of gravitational waves from coalescing binaries},
	Volume = {44},
        Pages = {3819-3824},
	Year = {1991}}


@article{Blackburn:2008rt,
	Author = {L. Blackburn and others},
	Date-Added = {2009-03-26 14:39:33 -0400},
	Date-Modified = {2009-03-26 14:40:50 -0400},
	Journal = {Class. Quant. Grav.},
	Number = {18},
	Title = {The LSC Glitch Group: Monitoring Noise Transients during the fifth LIGO Science Run},
	Volume = {25},
        Pages = {184004},
	Year = {2008}}


@article{Sadowski:2008vq,
	Author = {Aleksander Sadowski and Kryzsztof Belczynski and Tomasz Bulik and Natalia Ivanova and Frederic A. Rasio and Richard O'Shaughnessy},
	Date-Added = {2009-03-26 14:51:31 -0400},
	Date-Modified = {2009-08-14 10:38:25 -0400},
	Journal = {The Astrophysical Journal},
	Number = {2},
	Pages = {1162-1169},
	Title = {The Total Merger Rate of Compact Object Binaries in the Local Universe},
	Volume = {676},
	Year = {2008},
	Bdsk-Url-1 = {http://www.iop.org/EJ/abstract/0004-637X/676/2/1162}}


@article{OLeary:2007md,
	Author = {Ryan M. O'Leary and Richard O'Shaughnessy and Frederic A. Rasio},
	Date-Added = {2009-03-26 15:04:44 -0400},
	Date-Modified = {2009-03-26 15:05:43 -0400},
	Journal = {Phys. Rev. D},
	Number = {6},
	Title = {Dynamical Interactions and the Black Hole Merger Rate of the Universe},
	Volume = {76},
        Pages = {061504},
	Year = {2007}}


@article{Fregeau:2006lz,
	Author = {John M. Fregeau and Shane L. Larson and M. Coleman Miller and Richard O'Shaughnessy and Frederic A. Rasio},
	Date-Added = {2009-03-26 15:21:07 -0400},
	Date-Modified = {2009-03-26 15:24:52 -0400},
	Journal = {Astrophysical Journal},
	Number = {2},
	Title = {Observing the IMBH-IMBH Coalescence via Gravitational Radiation},
	Volume = {646},
        Pages = {L135-L138},
	Year = {2006}}



@article{Abbott:2009bh,
	Author = {B. Abbott and et al.},
	Date-Added = {2009-03-26 15:34:12 -0400},
	Date-Modified = {2009-08-03 13:29:04 -0400},
	Journal = {Phys. Rev. D},
	Number = {12},
	Pages = {122001},
	Title = {Search for gravitational waves from binary inspirals in the First Year of LIGO's S5 Data},
	Volume = {79},
	Year = {2009}}


@article{LSC:2008cq,
	Author = {Keita Kawabe for the LSC},
	Date-Added = {2009-04-03 12:19:37 -0400},
	Date-Modified = {2009-08-14 10:48:57 -0400},
	Journal = {Journal of Physics},
	Pages = {032003},
	Title = {Status of LIGO},
	Volume = {120},
	Year = {2008}}


@article{LSC:2006sf,
	Author = {Lisa M. Goggin for the LSC},
	Date-Added = {2009-04-10 12:14:18 -0400},
	Date-Modified = {2009-04-10 12:15:59 -0400},
	Journal = {Class. Quant. Grav.},
	Number = {19},
	Title = {Search for black hole ringdown signals in LIGO S4 data},
	Volume = {23},
        Pages = {S709-S713},
	Year = {2006}}

@article{Collaboration:2007sf,
	Author = {LIGO Scientific Collaboration and K Hurley},
	Date-Added = {2009-04-23 11:04:07 -0400},
	Date-Modified = {2009-04-23 11:05:48 -0400},
	Journal = {Astrophysical Journal},
	Number = {2},
	Title = {Implications for the Origin of GRB 070201 from LIGO Observations},
	Volume = {681},
        Pages = {1419-1430},
	Year = {2007}}

@article{Damour:2008sf,
	Author = {Thibault Damour and Alessandro Nagar},
	Date-Added = {2009-04-29 10:37:47 -0400},
	Date-Modified = {2009-04-29 10:39:18 -0400},
	Journal = {Phys. Rev. D},
	Number = {2},
	Title = {Comparing Effective-One-Body gravitational waveforms to accurate numerical data},
	Volume = {77},
        Pages = {024043},
	Year = {2008}}


@article{Buonanno:2007sf,
	Author = {Alessandra Buonanno and Yi Pan and John G. Baker and Joan Centrella and Bernard J. Kelly and Sean T. McWilliams and James R. van Meter},
	Date-Added = {2009-04-30 16:40:13 -0400},
	Date-Modified = {2009-04-30 16:41:47 -0400},
	Journal = {Phys. Rev. D},
	Number = {10},
	Title = {Approaching faithful template for nonspinning binary black holes using the effective-one-body approach},
	Volume = {76},
        Pages = {104049},
	Year = {2007}}
	
	
@article{Shoemaker:2008sf,
	Author = {Deidre Shoemaker and Birjoo Vaishnav and Ian Hinder and Frank Hermann},
	Date-Added = {2009-05-14 10:51:56 -0400},
	Date-Modified = {2009-05-14 10:53:29 -0400},
	Journal = {Class. Quant. Grav.},
	Number = {11},
	Title = {Numerical relativiy meets data analysis: spinning binary black hole case},
	Volume = {25},
        Pages = {114047},
	Year = {2008}}

	

@article{Vaishnav:2007ws,
	Author = {Birjoo Vaishnav and Ian Hinder and Frank Hermann and Deidre Shoemaker},
	Date-Added = {2009-05-14 11:04:16 -0400},
	Date-Modified = {2009-05-14 11:05:33 -0400},
	Journal = {Phys. Rev. D},
	Number = {8},
	Title = {Matched filtering of numerical relativity templates of spinning binary black holes},
	Volume = {76},
        Pages = {084020},
	Year = {2007}}
	
	
@article{Acernese:2009sf,
	Author = {F Acernese and others},
	Date-Added = {2009-05-22 09:39:31 -0400},
	Date-Modified = {2009-05-22 09:41:57 -0400},
	Journal = {Class. Quant. Grav.},
	Number = {8},
	Title = {Gravitational wave burst search in the Virgo C7 data},
	Volume = {26},
        Pages = {085009},
	Year = {2009}}
	
	
@article{LIGO:2009pz,
	Author = {LIGO Scientific Collaboration},
	Date-Added = {2009-05-22 09:44:44 -0400},
	Date-Modified = {2009-05-22 09:49:08 -0400},
	Journal = {arXiv:0905.0020},
	Title = {Search for gravitational-wave bursts in the first year of the fifth LIGO science run},
	Url = {http://arxiv.org/abs/0905.0020},
	Urldate = {May 22, 2009},
	Year = {2009}}




